Design and Implementation of Linked Planning Domain Definition Language

Planning is a critical component of any artificial intelligence system that concerns the realization of strategies or action sequences typically for intelligent agents and autonomous robots. Given predefined parameterized actions, a planning service should accept a query with the goal and initial state to give a solution with a sequence of actions applied to environmental objects. This paper addresses the problem by providing a repository of actions generically applicable to various environmental objects based on Semantic Web technologies. Ontologies are used for asserting constraints in common sense as well as for resolving compatibilities between actions and states. Constraints are defined using Web standards such as SPARQL and SHACL to allow conditional predicates. We demonstrate the usefulness of the proposed planning domain description language with our robotics applications.

==> sections/implementation-original.tex <==
%\section{Implementation}
%\label{sec:implementation}
\subsection*{Implementation}
\label{ssec:implementation}

In logic, the term decidable refers to the decision problem, the question of the existence of an effective method for determining membership in a set of formulas, or, more precisely, an algorithm that can and will return a boolean true or false value that is correct (instead of looping indefinitely, crashing, returning "don't know" or returning a wrong answer). Logical systems such as propositional logic are decidable if membership in their set of logically valid formulas (or theorems) can be effectively determined.

A theory (set of sentences closed under logical consequence) in a fixed logical system is decidable if there is an effective method for determining whether arbitrary formulas are included in the theory. Many important problems are undecidable, that is, it has been proven that no effective method for determining membership (returning a correct answer after finite, though possibly very long, time in all cases) can exist for them.
Many reasoners use first-order predicate logic to perform reasoning; inference commonly proceeds by forward chaining and backward chaining.

% https://en.wikipedia.org/wiki/Second-order_logic

%Forward chaining, tabled backward chaining 

%repeated application of modus ponens

%monotonic

%restriction 


% term 

\begin{algorithm}[t]
	\caption{Symbol Translation Map Construction for Alias Canonicalization}
	\label{alg:alias}
	\scriptsize
	\begin{algorithmic}
		\State \textbf{In}: a PDDLS Problem and PDDLS Domains
		\State \textbf{Out}: a set of symbol translation maps
				$\{ {\text{Map}}^{d}_{\text{symbol}\mapsto\text{symbol}} | d \in \text{PDDLS Domains} \}$
		\hspace{0.5cm}\\
		\State Initialize maps ${\text{Map}}_{\text{symbol}\mapsto\text{URI}}$  and
				${\text{Map}}_{\text{URI}\mapsto\text{symbol}}$ to be empty. 
				
		\For{each term definition entry in a PDDLS Problem $p$'s JSON-LD context}
			\State let $t$ and $u$ be a term and an IRI in the term definition, respectively
			
			\State add $t \mapsto u$  to ${\text{Map}}_{\text{symbol}\mapsto\text{URI}}$ 
			
			\State add $u \mapsto t$  to ${\text{Map}}_{\text{URI}\mapsto\text{symbol}}$
					if ${\text{Map}}_{\text{URI}\mapsto\text{symbol}}$ doesn't contain the key $u$
		\EndFor
		
		\For{each PDDLS domain $d$}
		\State Initialize a map ${\text{Map}}^{d}_{\text{symbol}\mapsto\text{symbol}}$  to be empty
		\For{each term definition entry in the PDDLS Domain $d$'s JSON-LD context}
		\State let $t$ and $u$ be a term and an IRI in the term definition, respectively

		\If{${\text{Map}}_{\text{symbol}\mapsto\text{URI}}$  has an entry $u \mapsto t$}
			% common URI and local symbol name
			\State add $t \mapsto t$  to ${\text{Map}}^{d}_{\text{symbol}\mapsto\text{symbol}}$ 
		\ElsIf{${\text{Map}}_{\text{URI}\mapsto\text{symbol}}$  contains the key $u$}
			\State let $t'$ be the value of ${\text{Map}}_{\text{URI}\mapsto\text{symbol}}$ for a key $u$
			\State add $t \mapsto t'$  to ${\text{Map}}^{d}_{\text{symbol}\mapsto\text{symbol}}$ 
		\Else
			% a first URI
			\If{${\text{Map}}_{\text{symbol}\mapsto\text{URI}}$  doesn't contain the key $t$}
				% a new local symbol name
				\State add $t \mapsto u$  to ${\text{Map}}_{\text{symbol}\mapsto\text{URI}}$ 
				\State add $u \mapsto t$  to ${\text{Map}}_{\text{URI}\mapsto\text{symbol}}$
				\State add $t \mapsto t$  to ${\text{Map}}^{d}_{\text{symbol}\mapsto\text{symbol}}$ 
			\Else
				% conflicting symbol name
				\State pick up a new key $t'$ not in ${\text{Map}}_{\text{symbol}\mapsto\text{URI}}$
				\State add $t' \mapsto u$  to ${\text{Map}}_{\text{symbol}\mapsto\text{URI}}$ 
				\State add $u \mapsto t'$  to ${\text{Map}}_{\text{URI}\mapsto\text{symbol}}$
				\State add $t \mapsto t'$  to ${\text{Map}}^{d}_{\text{symbol}\mapsto\text{symbol}}$ 
			\EndIf		
		\EndIf
		
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}


==> sections/introduction_reasoning.tex <==
\section{Introduction}
\label{sec:introduction}

Given a knowledge base and two logical instances $a$ and $b$, such as a peg and a hole, we often want to know if a role assertion axiom $(a, b):R$, such as the insertability of the peg into the hole, stands.  In practice, it is useful if the knowledge base can come from multiple separate sources for the same domain.  For example, in addition to a "static" ontology database as the common sense in the domain, such as the general knowledge of the "insertability", we would obtain a new information in the environment, such as pegs and holes and its instant properties such as shapes and sizes of them.  While this simple but tough research question of "common sense" was addressed in "Good Old-Fashioned Artificial Intelligence", or the symbolic AI paradigm until the late 1980s~\cite{Lenat:CACM1995:CYC}, but is not really focused on in Semantic Web studies.

While the underlying foundation of Description Logic (DL) gives a clear formalism and reasoning simplicity about OWL-based ontologies, the limitation of expressive power can be sometimes prohibitive in practice, in providing modular ontologies.
Actually, the authors experienced this problem in building cognitive robots~\cite{Munawar:ICRA2018:MaestROB} supported by a common sense knowledge base using Semantic Web technologies such as JSON-LD, RDF, and OWL.
In this paper, we propose a role-constructive reasoning, which allows to find relationships (roles in the DL terms) between unknown individuals, based on a predefined set of axioms.  In order to avoid computational complexity due to higher-order reasoning, meta-circularity is excluded in the proposed interpretation.
%SPARQL and SHACL, as the standard graph examination languages, are employed to allow powerful expression of role construction.

%\cite{Rudolph:KR2016:undecidability}

%P(A, B) and Q(A, B) and S(P, Q) then R(A, B)

\topic{Making robot programming easy.}
Modular componentization of robotic cognition and action systems is a key for ease-of-programming of cognitive robots or agents, which interact with human to perform complicated tasks.
A robot may listen to an instruction from a human user, see peg and hole objects on a table, and perform the sophisticated combination of pick, place, insert and other actions to satisfy the instructed goal, such as ``Fill up all the holes.''
A component called {\it{``planner''}} usually plays the orchestration role in robotic systems~\cite{Ghallab:2016:AutomatedPlanning}, accepting the goal and initial state as a problem, and actions available as a domain, to give a sequence of actions to solve the problem.
Cognitive solutions of visual recognition and natural language processing are getting well componetized and are even available as off-the-shelf Web services (or APIs) 
\cite{Waibel:2011:roboearth}\cite{Kehoe:ToASE2015:cloudroboticssurvey} to obtain such the goals and initial states.

\topic{Skill repository does not scale with PDDL.}
Unfortunately, the componentization of actions in the sense of Web-scale have not yet been established to be readily available.
Ideally, each type of actions should have been available on the Web, with previously machine-trained or hand-configured models to control row-level robot actuations such as changing the joint angles of robot arms.
The exchangeable formats of machine-trained models such as PMML and PFA~\footnote{\url{http://dmg.org/pmml/products.html}},  or more recently neural model-dedicated ONNX~\footnote{\url{http://onnx.ai}} have been used or getting standardized.
However, though PDDL~\cite{McDermott:1998:PDDL,Fox:JAIR2003:PDDL21} is a de facto standard in the Artificial Intelligence for providing commonly-understandable planning problems with well-simplified metadata for actions, it is not designed to be used as metadata suitable for indexing such models as actions in a web-scale. 

\topic{PDDL with semantics to expect helps from Semantic Web technologies.}
This paper introduces the PDDLS language and a reference design and implementation of its resolver.  PDDLS has a minimal extension from PDDL~\cite{McDermott:1998:PDDL,Fox:JAIR2003:PDDL21} to help planning domain descriptions to interoperate at Web-scale, leveraging Semantic Web technologies and assets~\cite{Horrocks:2008:OntoSemWeb}.  While sharing the namespace concept found in Web-PDDL~\cite{Dou:2005:OntEngine} or  PDDL/M~\cite{dornhege2012semantic}, PDDLS follows the practical annotation design of JSON-LD~\cite{Lanthaler:WSREST2012:JSONLD} to allow annotating any local symbols or terms to be bound to globally unique IDs, IRIs, which can be resolved using Semantic Web~\cite{Shadbolt:2006:semanticweb} technologies.  Also, an additional reasoning step supported by Semantic Web technologies, if working well, would help a planner-like system to integrate actions developed by multiple vendors or communities.
In this research we develop a knowledge-driven engine to give robots the power of processing the common sense knowledge which helps for better understanding of human commands.

%\topic{OWL-style TBox (subclass) knowledge common sense can help.}
%Knowledge described using  OWL can help robots to understand whether a command is meaningful to process. Let's assume o1 is-an Object.  o2 is-a Pyramid.  Any object cannot-be-on-top-of any object in SharpHeadObject (ABox). Pyramid is-subclass-of SharpHeadObject. (TBox), because of that o1 cannot-be-on-top-of o2. From the perspective of giving the command “Put something on top of another thing”, the robot needs to know which objects can be put on top of another. For example, “Put the book on the table” is a meaningful command which a robot may be able to execute. However, “Put the book on the pyramid” is not a meaningful command as the robot will not be able to do that due to physical constraints.  

The advantage of this approach is that we do not need to define grammar like ELI did to achieve similar task ~\cite{connell2014extensible}. As our approach is using ontology we can update the knowledge at runtime, which makes the system easily extendable to handle complex scenarios. Even though, here we considered only the orientation and the relationship of the objects to be able to put in top of one and another. It can be extended for any other required restrictions using ontology.

\topic{Help from OWL-style common sense is limited as we need to handle objects unknown at the time of KB creation.}
By using the knowledge and ontology of physical constraints and relationships, these abstractions allow the grounding of human instructions to actionable commands. 
The framework performs symbolic reasoning at higher level, which is important for long term autonomy and to make the whole system accountable for its actions.
Individual skills are allowed to use machine learning or rule based systems.
We provide a mechanism to extend the framework by developing new services or connecting it with other robot middlewares and scripting languages.
This allows the higher level reasoning to be done using PDDL (Planning Domain Definition Language) planner with proposed extension, while the lower level skills can be executed as ROS (Robotics Operating System) nodes.

Lack of common sense knowledge is a significant issue to communicate with robots.
In this research we develop a knowledge-driven engine to give robots the power of processing the common sense knowledge which helps for better understanding of human commands.
In our approach, at first, the input command given in natural language is parsed using a Natural Language Understanding service, which identifies the action, subject and object.
Then the system matches action and pattern with the list of skills available for the robot. The robot has a model database and a list of objects remaining in front from its sensors. From that list it will able to find the subject and object positions. From the model database it can find the object type and from the ontology the robot can check whether the subject can be put on top of the object. If it is not valid then robot will inform the user that the command cannot be performed. If it is valid then, the robot will perform the put operation.

%\topic{We demonstrate its effectiveness in a practical robotics use case.}
%We show the capabilities of the framework by a scenario where a human teaches a task to a communication robot (Pepper~\cite{url:pepper}) by demonstration.
%The robot understands the tasks and collaborates with an industrial manipulator (UR5~\cite{url:ur5}) to execute the task, using the action primitives that UR5 has previously acquired by learning or programming.
%The industrial robot has the ability to perform physical manipulation, but it lacks the key sensors that can help in a particular situation (e.g. error recovery etc.).
%In the scenario, the communication robot having these sensors can analyze and convert the plan to a command sequence for the robotic arm.
%Semantic ontologies are used to resolve the plan.

A second-order description logics~\cite{Szalas:2006:SecondOrderDL,Giacomo:AAAI2011:HigherOrderDL}.

This paper explores how semantic ontologies can help resolving semantically annotated problem as goals and initial states with semantically annotated actions with precondition and effects.  As what we can do with simple OWL 2 semantics resolvers is quite limited, we extend the PDDLS resolver to provide beyond the level of First-Order Description Logics, provided by OWL 2.  The extension involves the Second-Order Description Logics, which is generally hard to resolve, but we design it to be practically resolvable with a simple resolver implementation.  We also leverages some of standard semantic Web technologies: RDF, OWL, JSON-LD, SPARQL, and SHACL.

\topic{Contribution.}
The main contributions of this paper are:
\begin{description}
	\item[PDDLS design and implementation] We extended PDDL leveraging the JSON-LD.  A simple PDDLS-to-PDDL translator has been designed and implemented leveraging semantic technologies.
	\item[PDDLS semantics] To overcome the limitation with OWL with typical Descriptive Logic (DL) resolvers, we extend the DL with a powerful role construction operator.  The extended resolver for the operator is formally defined.
	\item[Demonstration with a robotics use case.] PDDLS usage in an actual robotics scenario has been shown with a working cognitive robot system.
\end{description}

%Starting from Section~\ref{sec:motivation} to detail the motivation behind the work, the rest of the paper is organized as follows.
%Section~\ref{sec:pddls} proposes the PDDLS language with syntax and semantics.
%Section~\ref{sec:semantics} discusses the resolver of PDDLS.
%In Section~\ref{sec:motivation}, We demonstrate how it can be used in our actual Robotics application, shown in Section~\ref{sec:motivation}.
%After discussing related work in Section~\ref{sec:relatedwork}, we conclude the paper with Section~\ref{sec:conclusion}.
The rest of this paper is organized as follows.  We start from the section describing a motivation behind the work and then we propose the PDDLS language with its syntax and semantics.
Then we discuss semantic resolvers for PDDLS in terms of expressive power.
We demonstrate how it can be used in our actual Robotics application, in the following section.
After mentioning related work, we conclude the paper.

==> sections/standards.tex <==
\subsection{Standards}
\label{ssec:standards}

While not universally adopted in the same way as SQL was for relational	databases, there are some standardization efforts such as SPARQL~\footnote{http://www.w3.org/TR/rdf-sparql-query/}~\cite{Perez:ToDS2009:SPARQL}, Gremlin~\footnote{http://tinkerpop.apache.org}~\cite{Rodriguez:DBPL2015:Gremlin} and Cypher~\footnote{http://www.opencypher.org}~\cite{Marton:ADBIS2017:opencypher}, leading to multi-vendor query languages.
